A Polynomial-time Bicriteria Approximation Scheme for Planar Bisection

Given an undirected graph with edge costs and node weights, the minimum bisection problem asks for a partition of the nodes into two parts of equal weight such that the sum of edge costs between the parts is minimized. We give a polynomial time bicriteria approximation scheme for bisection on planar graphs. Specifically, let $W$ be the total weight of all nodes in a planar graph $G$. For any constant $\varepsilon > 0$, our algorithm outputs a bipartition of the nodes such that each part weighs at most $W/2 + \varepsilon$ and the total cost of edges crossing the partition is at most $(1+\varepsilon)$ times the total cost of the optimal bisection. The previously best known approximation for planar minimum bisection, even with unit node weights, was $O(\log n)$. Our algorithm actually solves a more general problem where the input may include a target weight for the smaller side of the bipartition.

==> DP.tex <==
\section{Dynamic program}
\label{sec:DP}

There is a standard dynamic programming algorithm for computing an optimal
$b$-bipartition in a graph $H$ with branchwidth~$k$. For each subset $X$ of
edges in the minimum width branch decomposition of $H$, for each subset $A$ of
the boundary vertices $\partial
X$ of $X$, and for each possible weight $w\in \{0,1, \dots, W\}$, the
dynamic program stores the minimum cost of a bipartition $(S,\bar S)$
such that the weight of $S$ is exactly $w$ and $\partial X \cap S = A$.  
The number of configurations for a single subset of edges~$X$ is thus $W2^{O(k)}$, 
and the running time of the dynamic program is $n W^2 2^{O(k)}$.
Our approximation framework runs this dynamic program on a graph of branchwidth~$k = O(\eps^{-7}
\log W)$, making the overall running time equal to $n W^2 2^{O(\eps^{-7} \log W)}$.


==> no_red_cycles.tex <==
\iffalse
Basic idea:

Skip the red-cycle step.

Each time the algorithm chooses a blue cycle C to include in the
skeleton, it assigns to C all the faces that are charged to that
cycle.  Ordinarily all faces enclosed by C are included.  However, in
the region resulting from a splicing step, the faces enclosed by the
leafward cycle in the splice-pair are merged to a single face that is
assigned zero weight.  Let F be this set of faces.  If subsequently a
cycle C is selected to include in the skeleton, the faces in F are not
assigned to C even if C encloses them.

There is still a tree associated with the set of cycles in the
skeleton but it is defined slightly differently: C1 is a descendant of
C2 if the set of faces assigned to C1 is a subset of the set of faces
assigned to C2.

The splicing step is as before: If a splice is done involving C0 and
C1, all descendants of C0 that are not descendants of C1 are removed.

We can show that once a splice takes place from C0 to C1 then the edge
in the tree between them remains in place for the remainder of the
algorithm.

Each non-splicing step adds one node to the tree of cycles.  The tree
of cycles never contains more than O(n) nodes, where n is the number
of faces.  Each splicing step makes one edge permanent.  Therefore the
number of iterations is O(n^2).

The weight argument goes as before.  When the algorithm terminates,
the depth of the tree is O(log n).  Each node in the tree
corresponds to a cycle that charged to a set of faces, and each face
is charged to at most O(log n) times, so the total charge is O(log n)
times the total face weight.
\fi

\note{the following belongs in the prelims}
\paragraph{Regions defined by non-crossing sets of cycles}
A set $S$ of sets is non-crossing if for every two sets $A,B \in S$,
either $A \cap B = \emptyset$ or $A \subseteq B$ or $B \subseteq A$.
Our algorithm maintains a set $\mathcal C$ of non-crossing simple 
cycles. Along the execution cycles are added or removed from $\mathcal
C$. 
The cycles of $\mathcal C$ partition $G$ into {\em regions}. The
cycles bounding a region $R$ are called the {\em boundary} of
$R$. Among the boundary cycles of $R$, a single one, called the {\em
outer boundary} of $R$, encloses all the others, which are called the
{\em holes} or $R$. An edge of $R$ that does not
belong to the boundary of $R$ is said to be {\em strictly internal}
to $R$.

\note{PK: This definition is somewhat problematic since it doesn't include
  the outer boundary face.  Where is the definition used?}
Similarly, for a subset $R$ of faces of $G$, the boundary of $R$
consists of the set $\mathcal C$ of cycles such that $R$ is exactly the set of
faces enclosed by $\mathcal C$.
For any region~$R$ and cycle~$C$ not crossing any member of~$\mathcal{C}$,
we say~$C$ belongs to region~$R$ if all the edges of~$C$ belong to
~$R$ and if $C$ is not a hole of $R$.
By this definition, each cycle~$C$ not crossing any member
  of~$\mathcal{C}$ belongs to exactly one region.

At the time a cycle $C$ is added to $\mathcal C$ it is associated with
the set $F(C)$ of faces in the new region whose outer boundary is
$C$. 
Note that while the region whose outer boundary is $C$ may subsequently
change as cycles are added to and removed from $\mathcal C$, the set
$F(C)$ is determined at the time $C$ is added to
$\mathcal C$, and remains fixed.

The set $\mathcal C$ can be represented by a rooted tree $\mathcal
T$ as follows. Every node $v \in \mathcal T$ corresponds to a 
cycle $C_v \in \mathcal C$. 
Ancestry in $\mathcal T$ is determined by the subset relation of the
associated sets $F(C)$ of faces:
Node $v$ is an ancestor of node $u$ in $\mathcal T$ if $F(C_u)
\subseteq F(C_v)$. Abusing notation, we say that $C_v$ is an ancestor
of $C_u$ in $\mathcal T$ if $u$ is an ancestor of $v$ in $\mathcal T$.

\note{The following belongs to the skeleton section}
The algorithm constructs a family~$\mathcal C$ of mutually noncrossing
cycles, which includes  the outer
face~$f_\infty$.  We refer to $\mathcal C$ as the \emph{skeleton}.

\begin{algorithm} \caption{Skeleton$(G)$}
\label{alg:skeleton}
\begin{algorithmic}[1]
\STATE $\mathcal C \leftarrow \set{f_\infty}$
\WHILE{$\exists$ region $R$ and cycle $C'$ in $R$
  s.t. $\ratio_R(C') \leq \epsilon^{-1} \lambda$ and $C'$ has an edge
  strictly in~$R$ %one edge of~$C'$ is strictly in~$R$
  \textbf{or}
  $\exists$ a leafward path~$Q = C_0, C_1, \dots, C_i$ in~$\mathcal{T}$
  s.t. $i\geq 2$, and $w(F(C_0)) \leq (1+\eps^2)w(F(C_i))$} \label{line:while-blue}
  \IF{$\exists$ region $R$ and cycle $C'$ in $R$ and 
$C'$ has an edge strictly in~$R$  %one edge of~$C'$ is strictly in~$R$
    s.t. $\ratio_R(C') \leq \epsilon^{-1} \lambda$} \label{line:if-blue}
    \STATE  let $C$ be a \textbf{maximally} face enclosing cycle in $R$
    s.t. $\ratio_R(C) \leq \epsilon^{-1} \lambda$ and $C$ has an edge
  strictly in~$R$ %one edge of~$C'$ is strictly in~$R$
    \label{line:find-blue}
    \STATE add $C$ to $\mathcal C$ \label{line:add-blue}
    \STATE set $F(C)$ to be the set of faces of $R$ enclosed by $C$
  \ELSE
    \STATE let $Q = C_0, C_1, \dots, C_i$ be a maximal leafward path in $\mathcal T$
    s.t. $i\geq 2$, and 
    $w(F(C_0)) \leq (1+\eps^2)w(F(C_i))$, and
    $C_0$ has the least depth in~$\mathcal{T}$ for any such sequence \label{line:Q}
    \WHILE {$\exists$ child~$C \neq C_i$ of~$C_0$} \label{line:splice}
      \STATE remove $C$ from~$\mathcal{C}$ \COMMENT{Splicing step.}
    \ENDWHILE
  \ENDIF
\ENDWHILE
\STATE return $\mathcal{C}$
\end{algorithmic}
\end{algorithm}

\begin{lemma}\label{lem:leaf}
Let $C_v$ be a leaf of $\mathcal T$ just before a splicing step at
time $t$. Then
$C_v$ remains a leaf and is never removed from $\mathcal T$. Moreover,
for any subsequent cycle $C_u$
added to $\mathcal C$, $C_u$ cannot be an ancestor of $C_v$.
\end{lemma}
\begin{proof}
Let $R_v$ be the region whose outer boundary is $C_v$ at time $t$.
Since $C_v$ is a leaf of $\mathcal T$, the faces in $R_v$, the
faces enclosed by $C_v$ and $F(C_v)$ are all the same set.

Since a splicing step occurs only if no cycle can be added to
$\mathcal C$, no cycle in $R_v$ can be added to $\mathcal C$ at time $t$.
Since a splicing step never deletes a leaf of $\mathcal T$ nor does it affect any
region whose outer boundary is a leaf of $\mathcal T$, no cycle in $R_v$
can be added to $\mathcal C$ after time $t$ as well. It
follows that $C_v$ is a leaf of $\mathcal T$ for the remainder of
the execution of the algorithm and hence $C_v$ remains a leaf of
$\mathcal T$ and is never removed.

Now consider any cycle $C_u$ that is added to $\mathcal C$ after time
$t$. From the discussion above, $C_u$ does not belong to $R_v$. Hence
$F(C_u)$ and $F(C_v)$ are disjoint, so $C_u$ is not an ancestor of
$C_v$ in $\mathcal T$.
\end{proof}

\begin{lemma}The skeleton algorithm runs in polynomial time.
\end{lemma}
\begin{proof}
Lemma~\ref{lem:leaf} implies that the number of leaves of $\mathcal T$
strictly increases between every two consecutive
splicing steps. Since
the total number of nodes in $\mathcal T$ at any given time is bounded by the number of
faces of $G$, which is $O(n)$, there are $O(n)$ splicing steps. Hence,
the total number of cycles added to $\mathcal
C$ throughout the execution of the skeleton construction algorithm is
$O(n^2)$. Since each cycle is found in polynomial time, the total
running time is polynomial.
\end{proof}





Since K is not in the skeleton, $c(K)/w_R(K) \geq
\eps^{-1}\lambda$. So $w_R(K) \leq \eps c(K) / \lambda$.
Similarly, Since $C'_i$ is not in the skeleton $w_R(C'_i) \leq \eps
c(K) / \lambda$. Hence $\Delta w(K) \leq \eps c(K) / \lambda$.
